Rule2Text: A Framework for Generating and Evaluating Natural Language Explanations of Knowledge Graph Rules

Knowledge graphs (KGs) can be enhanced through rule mining; however, the resulting logical rules are often difficult for humans to interpret due to their inherent complexity and the idiosyncratic labeling conventions of individual KGs. This work presents Rule2Text, a comprehensive framework that leverages large language models (LLMs) to generate natural language explanations for mined logical rules, thereby improving KG accessibility and usability. We conduct extensive experiments using multiple datasets, including Freebase variants (FB-CVT-REV, FB+CVT-REV, and FB15k-237) as well as the ogbl-biokg dataset, with rules mined using AMIE 3.5.1. We systematically evaluate several LLMs across a comprehensive range of prompting strategies, including zero-shot, few-shot, variable type incorporation, and Chain-of-Thought reasoning. To systematically assess models' performance, we conduct a human evaluation of generated explanations on correctness and clarity. To address evaluation scalability, we develop and validate an LLM-as-a-judge framework that demonstrates strong agreement with human evaluators. Leveraging the best-performing model (Gemini 2.0 Flash), LLM judge, and human-in-the-loop feedback, we construct high-quality ground truth datasets, which we use to fine-tune the open-source Zephyr model. Our results demonstrate significant improvements in explanation quality after fine-tuning, with particularly strong gains in the domain-specific dataset. Additionally, we integrate a type inference module to support KGs lacking explicit type information. All code and data are publicly available at https://github.com/idirlab/KGRule2NL.

==> sec-rule.tex <==
\section{Rule Selection from Knowledge Graphs}\label{sec:rules}
\subsection{Rule Mining Algorithm}
We employed AMIE 3.5.1, a well-established rule learning system in its latest version, due to its comprehensive metrics for rule evaluation as well as its proven compatibility with our chosen benchmark datasets. In AMIE, a rule has a body (antecedent) and a head (consequent), represented as $B_1 \land B_2 \land \ldots \land B_n \Rightarrow H$
, or in simplified form \(\overrightarrow{B} \Rightarrow H\).  
The body consists of multiple \textit{atoms} $B_1$, $\ldots$, $B_n$ and the head $H$ itself is also an atom. In an atom \rel{r}(\entity{h},\entity{t}), which is another representation of a triple \triple{h}{r}{t}, the subject and/or the object are variables to be instantiated. The prediction of the head can be carried out when all the body atoms can be instantiated in the KG. In AMIE, the concept of \textit{support} quantifies the amount of evidence (i.e., correct predictions) for each rule in the data. It is defined as the number of distinct (subject, object) pairs in the head of all valid instantiations of the rule in the KG. The concept of \textit{head coverage}, a proportional version of \textit{support},  is the fraction of \textit{support} over the number of facts in relation \rel{r}, where \rel{r} is the relation in the head atom. The \textit{standard confidence} of a rule is the fraction of \textit{support} over the number of instantiations of the rule body. To mine the rules, we used the default settings of AMIE for optimized performance, with minimum thresholds of 0.1 for \textit{head coverage} and \textit{standard confidence}, and a maximum threshold of 3 for the number of atoms.\todo{EXAMPLES whole paper} 

\subsection{Datasets}
For our experiments, we leveraged three datasets. FB15k-237, a small subset of the Freebase dataset, was selected as it is a widely used benchmark for KG completion, recognized for avoiding the data leakage issues of FB15k~\cite{bordes2013translating}. Its multi-domain coverage makes it well-suited for extracting logical rules with diverse relations. FB-CVT-REV and FB+CVT-REV~\cite{shirvani2023comprehensive} datasets (Statistics shown in Table~\ref{tab:datastat}) are large-scale variants of the Freebase dataset designed to eliminate the data leakage issue previously identified in FB15k. FB+CVT-REV includes mediator entities (i.e., Compound Value Type nodes) originally present in Freebase to represent n-ary relations. In contrast, FB-CVT-REV converts n-ary relationships centered on a CVT node into binary relations by concatenating the edges that connect entities through the CVT node, a method also used in FB15k-237. As shown in Table~\ref{tab:datastat}, the conversion process has resulted in a higher number of rules in these two datasets compared to those in FB+CVT-REV. Including these datasets facilitates the analysis of large-scale data and the effects of mediator nodes and concatenated relationships on the derived rules and generated explanations.

The label of a concatenated relation is formed by merging the labels of two underlying relations. As a result, the label becomes lengthy, taking the format of \rel{domain1/type1/label1./domain2/type2/label2}. Notably, the domains and even types can sometimes be identical in concatenated labels, but label1 and label2 are always distinct. This format differs from the simpler structure of standard relations, which follow the format of \rel{domain/type/label}. Thus, this added complexity can pose a greater challenge for LLMs in generating natural language explanations.


